A Weighted Solution to SVM Actionability and Interpretability

Research in machine learning has successfully developed algorithms to build accurate classification models. However, in many real-world applications, such as healthcare, customer satisfaction, and environment protection, we want to be able to use the models to decide what actions to take. We investigate the concept of actionability in the context of Support Vector Machines. Actionability is as important as interpretability or explainability of machine learning models, an ongoing and important research topic. Actionability is the task that gives us ways to act upon machine learning models and their predictions. This paper finds a solution to the question of actionability on both linear and non-linear SVM models. Additionally, we introduce a way to account for weighted actions that allow for more change in certain features than others. We propose a gradient descent solution on the linear, RBF, and polynomial kernels, and we test the effectiveness of our models on both synthetic and real datasets. We are also able to explore the model's interpretability through the lens of actionability.

==> comparative.tex <==
Table \ref{tab:comparative} summarizes and compares the main characteristics of
{\sc Dakar} and the different approaches referenced
in Section \ref{related}. In this table, the term approach refers either to an
implanted system or to an algorithm.  These approaches are compared according
to:

\begin{itemize}
\item Knowledge extracted: The kind of actions discovered.
\item Model/domain knowledge: The model on which the method relies to discover actionable knowledge and the domain knowledge used.
\item Measures: The quality criteria used to discover and assess actionable knowledge.
\item Method: A brief description of the learning strategy of the approach detailed in Section \ref{related}.
\end{itemize}

\begin{table*}[]
{\footnotesize
  \begin{center}
    \begin{tabular}{p{0.4cm}|p{2.5cm}|p{1.6cm}|p{2.1cm}|p{1.4cm}|p{5.3cm}|}   \cline{2-6} 
       &{\bf Approach} & {\bf Knowledge extracted} & {\bf Model/domain knowledge} &  {\bf Measures} &  {\bf Method}\\ \cline{2-6} 
    \end{tabular}
     \begin{tabular}{|p{0.4cm}|p{2.5cm}|p{1.6cm}|p{2.1cm}|p{1.4cm}|p{5.3cm}|}  \hline 
    \multirow{14}*{\rotatebox{90}{\large  Predefined actions}}
        &{\sc Kefir} [\cite{Shapiro94}]  & corrective actions& corrective actions & deviation, impact of deviation, interestingness  & Compute deviations according to the norms, order them using interestingness/impact measure, present key deviations, explanations and corrective actions in a written report. \\ \cline{2-6}
        &{\sc } [\cite{Adomavicius97}]  & actionable patterns& actionable patterns& - & Build an action tree, assign an actionable pattern to each node. Traverse the tree in order to get an insight about decisions to undertake.\\ \cline{2-6}
        & [\cite{eloviciB03}]  & actions & any classification model, actions & payoff& Use a classification system to classify an individual and then chose the action to do so as to maximize the expected payoff.\\ \cline{2-6}
        &[\cite{JiangWTF05}] & actionsets & influence matrix of actions on features & utility, actionability & Compute the new utility of an actionset on a population P using the utility on a role model of P. Partition data so as to maximize the actionability w.r.t. utility. \\ \hline\hline 
     \multirow{15}*{\rotatebox{90}{\large  Actionable rules identification}}
        &{\sc Subgroup Discovery} [\cite{Lavrac04}]   & descriptive rules & -  & coverage, weighted relative accuracy& Find rules conditions $\rightarrow$ target-class. Expert-guided subgroup discovery in TP/FP space to search the rules with a maximal {\em q} value computed using a user TP/FP-trade off function. \\ \cline{2-6}
        &{\sc FindNA} [\cite{Liu01}]  & association rules& association rules with a class-value on their right-hand sides& $\chi^2$, coverage, support&  Discard the more general rules using their specialized rules with higher quality. Before removing any general rule, check that it is not still a strong rule after removing the tuples covered by the specialized rules from the dataset.\\ \cline{2-6}
	&{\sc Opportunity Map} [\cite{Zhao2005ICDM,Zhao2005}]  &  - & associative classification rules (CBA) & - & Interactive visualization of attributes, classes, data and rules in a matrix. Drill-down visualization of cells. \\ & & & & &\\\hline\hline 
     \multirow{23}*{\rotatebox{90}{\large  Elaboration of actions}}
        &{\sc Dar and Dear} [\cite{Ras2000}]  & action rules &  decision rules, stable and flexible features & coverage& Consider all pairs of decision rules with contradicting conclusions and same values for all stable attributes to generate action rules.\\ %\cline{2-6}
        &{\sc Dear2} [\cite{Tsay2005}]  & action rules &  decision rules, stable and flexible features & coverage& Organize decision rules into equivalence subclasses. Consider only pairs of rules belonging to some equivalence subclasses to construct extended action rules. \\ \cline{2-6}
        &{\sc Proactive Solution} [\cite{Ling02}]  & action rules& decision trees & net profit& Build a decision tree modeling customers profiles. If a customer falls in an undesired leaf, search for the optimal actions that move the customer to another leaf.\\ \cline{2-6}
        & [\cite{Yang2002}]  & actions & case bases& cost, rank & Mining case bases to identify representative role models. Three approaches: instance-based, cluster-based and SVM-based. Switching plan generation where negative cases are switched to positive cases using actions suggested by role models. \\ \cline{2-6}
        %&{\sc SVM-CBMine} [\cite{Yang2002}]  & action & SVM vector extracted from data  & & Case-based reasoning\\ \cline{2-6}
	&{\sc Dakar} [\cite{trepos05}]  & actions & classification rules, weights of flexible features& coverage, quality, distance, benefit & Given an unsatisfactory situation and relying on a set of classification rules, discover a set of action recommendations that propose minimal changes to improve that situation.\\ \hline
    \end{tabular}
    \medskip
    \caption{Characteristics of the state-of-the-art methods for learning actionable knowledge}
    \label{tab:comparative}
  \end{center}
}
\end{table*} 

